Robust and Adaptive Sequential Submodular Optimization

Emerging applications of control, estimation, and machine learning, ranging from target tracking to decentralized model fitting, pose resource constraints that limit which of the available sensors, actuators, or data can be simultaneously used across time. Therefore, many researchers have proposed solutions within discrete optimization frameworks where the optimization is performed over finite sets. By exploiting notions of discrete convexity, such as submodularity, the researchers have been able to provide scalable algorithms with provable suboptimality bounds. In this paper, we consider such problems but in adversarial environments, where in every step a number of the chosen elements in the optimization is removed due to failures/attacks. Specifically, we consider for the first time a sequential version of the problem that allows us to observe the failures and adapt, while the attacker also adapts to our response. We call the novel problem Robust Sequential submodular Maximization (RSM). Generally, the problem is computationally hard and no scalable algorithm is known for its solution. However, in this paper we propose Robust and Adaptive Maximization (RAM), the first scalable algorithm. RAM runs in an online fashion, adapting in every step to the history of failures. Also, it guarantees a near-optimal performance, even against any number of failures among the used elements. Particularly, RAM has both provable per-instance a priori bounds and tight and/or optimal a posteriori bounds. Finally, we demonstrate RAM's near-optimality in simulations across various application scenarios, along with its robustness against several failure types, from worst-case to random.

==> SectionII.tex <==
\section{Problem Formulation}\label{sec:problem_statement}
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 


We formally define resilient monotone sequential maximization.  
We start with the basic definition of monotonicity.

%\begin{definition}[Monotonicity]\label{def:mon}
%Consider any finite ground set~$\calV$. The set function $f:2^\calV\mapsto \mathbb{R}$ is non-decreasing if and only if for any sets $\calA\subseteq \calA'\subseteq\calV$, it holds $f(\calA)\leq f(\calA')$.
%\end{definition}

We define next the main problem in this paper.

%\begin{problem}[Resilient Monotone Sequential Maximization]\label{pr:robust_sub_max} 
%Consider the parameters: an integer $T$; finite ground sets $\calV_1,\ldots,\calV_T$;
%a non-decreasing set function $f:2^{\calV_1}\times \cdots\times 2^{\calV_T} \mapsto \mathbb{R}$
%such that, without loss of generality, it holds $f(\emptyset)=0$ and $f$ is non-negative;
%finally, integers $\alpha_t$ and $\beta_t$ such that $0\leq\beta_t \leq \alpha_t \leq |\calV_t|$, for all $t=1,2,\ldots,T$\!.
% 
%The problem of \emph{resilient monotone sequential maximization} is to 
%maximize the objective function~$f$ through a sequence of~$T$ maximization steps, despite compromises to the solutions of each of the maximization steps; in particular, 
%at each maximization step $t=1,\ldots,T$ 
%a set $\calA_t\subseteq \calV_t$ of cardinality $\alpha_t$ is selected,
%and 
%is compromised by a worst-case set removal~$\calB_t$ of cardinality $\beta_t$.
%Formally:
%\vspace*{1mm}
%\begin{align*}
%\begin{split}
%\max_{\calA_1 \subseteq \calV_1}\min_{\;\calB_1 \subseteq \calA_1}&\cdots
%\max_{\calA_T \subseteq \calV_T}\min_{\;\calB_T \subseteq \calA_T} \; f(\calA_{1}\setminus \calB_1,\ldots,\calA_T\setminus \calB_T), \\
%%\vspace*{1mm}
%&\;\text{s.t. } \;\;\;|\calA_t|\;= \alpha_t, \;\; |\calB_t|\;\leq \beta_t, \;\;\; t=1,\ldots,T.
%\end{split}
%\end{align*}
%\end{problem}
%\medskip


As we mentioned in this paper's Introduction, Problem~\ref{alg:rob_sub_max} may be interpreted as a $T$-stage perfect information sequential game between two players~\cite[Chapter~4]{myerson2013game}, a ``maximization'' player, and a ``minimization'' player, who play sequentially, {both observing all past actions of all players}, and with the ``maximization'' player starting the game.  In the following paragraphs, we describe this game in more detail:
\begin{itemize}
\item \textit{1st round of the game in Problem~\ref{pr:robust_sub_max}}: the ``maximization'' player selects the set $\calA_1$; then, the ``minimization'' player observes $\calA_1$, and selects the set $\calB_1$ against $\calA_1$;
\item \textit{2nd round of the game in Problem~\ref{pr:robust_sub_max}}: the ``maximization'' player, who already knows $\calA_1$, observes $\calB_1$, and selects the set $\calA_2$, given $\calA_1$ and $\calB_1$; then, the ``minimization'' player, who already knows $\calA_1$ and $\calB_1$, observes $\calA_2$, and selects the set $\calB_2$ against $\calA_2$, given $\calA_1$ and $\calB_1$.

\begin{center}
$\vdots$
\end{center}

\item \textit{$T$-th round of the game in Problem~\ref{pr:robust_sub_max}}: the ``maximization'' player, who already knows the history of selections $\calA_1,\ldots, \calA_{T-1}$, as well as, removals $\calB_{1},\ldots, \calB_{T-1}$, selects the set $\calA_T$, given $\calA_1,\ldots, \calA_{T-1}$ and $\calB_{1},\ldots, \calB_{T-1}$; then, the ``minimization'' player, who also already knows the history of selections $\calA_1,\ldots, \calA_{T-1}$, as well as, removals $\calB_{1},\ldots, \calB_{T-1}$, observes $\calA_T$, and selects the set $\calB_T$ against $\calA_T$, given $\calA_1,\ldots, \calA_{T-1}$ and $\calB_{1},\ldots, \calB_{T-1}$.
\end{itemize} 

==> preamble_packages.tex <==
%!TEX root = main.tex

% LC: debug
%==========================================================================
%\usepackage{refcheck}
%\usepackage[notref]{showkeys}
%==========================================================================

% LC: to be used for TRO
%==========================================================================
% \usepackage{mathptmx} % assumes new font selection scheme installed
%\usepackage{times} % assumes new font selection scheme installed
%==========================================================================
\usepackage{comment}
\usepackage{siunitx}
\usepackage{relsize}
\usepackage{ifthen}

\usepackage[caption=false]{subfig}

% \begin{comment}
% % Fancy formatting 
% \usepackage[tracking=false,kerning=true,spacing=true]{microtype}
% \usepackage[caption=false]{subfig}

% \usepackage[style=numeric-comp,sorting=none,firstinits=true, maxnames=3,bibstyle=numeric,abbreviate=false,defernums=true,eprint=false,backend=bibtex]{biblatex}
% \renewcommand{\bibfont}{\footnotesize}
% % \DeclareFieldFormat[article]{pages}{#1}%
% % \DeclareFieldFormat[inproceedings]{pages}{#1}%

% \AtEveryBibitem{%
%   \ifentrytype{article}{%
%     \clearfield{pages}%
%   }{%
%   }%
%   \ifentrytype{inproceedings}{%
%     \clearfield{pages}%
%   }{%
%   }%
% }
% \end{comment}

% \bibliography{commons/bib/strings_long}
% \bibliography{commons/bib/all_only_one_w_pages}
% \bibliography{../../references/references}

% \usepackage[noadjust]{cite}
%\usepackage[vlined,ruled,linesnumbered]{algcompatible}
\usepackage{graphics} % for pdf, bitmapped graphics files
\usepackage{rotating}
\usepackage{color}
\usepackage{enumerate}
\usepackage[T1]{fontenc}
\usepackage{psfrag}
\usepackage{epsfig} % for postscript graphics files
%\usepackage{subfigure}
% \usepackage{hyperref}
\usepackage{booktabs}
\usepackage{graphicx,url}
\usepackage{multirow}
\usepackage{array}
\usepackage{latexsym}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage{amsthm}
\usepackage{xstring}
%\usepackage[noend]{algorithmic}
\usepackage{multirow}
\usepackage{xcolor}
\usepackage{prettyref}
\usepackage{flexisym}
\usepackage{bigdelim}
\usepackage{breqn} % load this last
\usepackage{listings}
\let\labelindent\relax
\usepackage{enumitem}
\usepackage{xspace}
\usepackage{bm}
\graphicspath{{./figures/}}
\usepackage{tikz}
\usetikzlibrary{matrix,calc}


%\usepackage{amsthm} % math
\usepackage{lineno}



%\usepackage{ifpdf}
% Heiko Oberdiek's ifpdf.sty is very useful if you need conditional
% compilation based on whether the output is pdf or dvi.
% usage:
% \ifpdf
%   % pdf code
% \else
%    dvi code
% \fi
% The latest version of ifpdf.sty can be obtained from:
% http://www.ctan.org/tex-archive/macros/latex/contrib/oberdiek/
% Also, note that IEEEtran.cls V1.7 and later provides a builtin
% \ifCLASSINFOpdf conditional that works the same way.
% When switching from latex to pdflatex and vice-versa, the compiler may
% have to be run twice to clear warning/error messages.

% *** GRAPHICS RELATED PACKAGES ***
%
%\ifCLASSINFOpdf
  % \usepackage[pdftex]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../pdf/}{../jpeg/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.pdf,.jpeg,.png}
%\else
  % or other class option (dvipsone, dvipdf, if not using dvips). graphicx
  % will default to the driver specified in the system graphics.cfg if no
  % driver is specified.
  % \usepackage[dvips]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../eps/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.eps}
%\fi


\usepackage{mdwlist}
\let\stditemize\itemize
\let\endstditemize\enditemize
\let\itemize\undefined
\makecompactlist{itemize}{stditemize}

%\let\stdenumerate\enumerate
%\let\endstdenumerate\endenumerate
%\let\enumerate\undefined
%\makecompactlist{enumerate}{stdenumerate}
 

